Generating Annotated High-Fidelity Images Containing Multiple Coherent Objects

Recent developments related to generative models have made it possible to generate diverse high-fidelity images. In particular, layout-to-image generation models have gained significant attention due to their capability to generate realistic complex images containing distinct objects. These models are generally conditioned on either semantic layouts or textual descriptions. However, unlike natural images, providing auxiliary information can be extremely hard in domains such as biomedical imaging and remote sensing. In this work, we propose a multi-object generation framework that can synthesize images with multiple objects without explicitly requiring their contextual information during the generation process. Based on a vector-quantized variational autoencoder (VQ-VAE) backbone, our model learns to preserve spatial coherency within an image as well as semantic coherency between the objects and the background through two powerful autoregressive priors: PixelSNAIL and LayoutPixelSNAIL. While the PixelSNAIL learns the distribution of the latent encodings of the VQ-VAE, the LayoutPixelSNAIL is used to specifically learn the semantic distribution of the objects. An implicit advantage of our approach is that the generated samples are accompanied by object-level annotations. We demonstrate how coherency and fidelity are preserved with our method through experiments on the Multi-MNIST and CLEVR datasets; thereby outperforming state-of-the-art multi-object generative methods. The efficacy of our approach is demonstrated through application on medical imaging datasets, where we show that augmenting the training set with generated samples using our approach improves the performance of existing models.

==> abstract.tex <==
Recent developments related to generative models have made it possible to generate diverse high-fidelity images. 
%Generally, these models assume a centralized object within an image or images from a specific domain or distribution.
In particular, layout-to-image generation models have gained significant attention due to their capability to generate realistic complex images containing distinct objects. 
These models are generally conditioned on either semantic layouts or textual descriptions. 
However, unlike natural images, providing auxiliary information can be extremely hard in domains such as biomedical imaging and remote sensing. 
In this work, we propose a multi-object generation framework\footnote{The code will be available atbuyh \href{https://github.com/Cynetics/MSGNet/}{https://github.com/Cynetics/MSGNet/} } that can synthesize images with multiple objects without explicitly requiring their contextual information during the generation process. 
Based on a vector-quantized variational autoencoder (VQ-VAE) backbone, our model learns to preserve spatial coherency within an image as well as semantic coherency between the objects and the background through two powerful autoregressive priors: PixelSNAIL and LayoutPixelSNAIL. 
While the PixelSNAIL learns the distribution of the latent encodings of the VQ-VAE, the LayoutPixelSNAIL is used to specifically learn the semantic distribution of the objects. 
%Further, through an added self-attention pathway in the VQVAE, our model can leverage from features located in even the farthest sections of any image. 
An implicit advantage of our approach is that the generated samples are accompanied by object-level annotations.
We demonstrate how coherency and fidelity are preserved with our method through experiments on the Multi-MNIST and CLEVR datasets; thereby outperforming state-of-the-art multi-object generative methods.  The efficacy of our approach is demonstrated through application on medical imaging datasets, where we show that augmenting the training set with generated samples using our approach improves the performance of existing models.
%Furthermore, we show that our proposed method can be used as a reliable generative modelling technique for data augmentation through the application on two medical imaging datasets.

==> broader_impact.tex <==
%We have proposed a generative modelling framework that is suited for images containing multiple distinct objects. We have experimentally validated on small datasets that our approach strongly adheres to the implicit spatial and semantic constraints of the training data. 
The framework proposed in this paper is suited for image generation process for a broad set of disciplines, and especially the safety-critical fields such as medical imaging, self driving. However, the disclaimer is that more work is needed to make this approach completely ready for such fields. Further, our approach is a deep learning-driven generative modelling process. Thus, similar to other approaches that learn from data, our approach runs the risk of producing biased samples. However, on the positive side, selective acceptance of the generated samples from our approach can help to reduce the inherent bias of the original data itself and reduce the effect of bias in other deep learning models through targeted data augmentation. The discriminative power of our approach can be improved significantly by replacing the current backbone autoencoder with more powerful frameworks.
%With this ability of controlling the generation process in a more direct way, we are able to generate specific instances of, for instance, medical cases for further study by students(??). 
Moreover, with a network that is sufficiently diverse and that produces images of high-fidelity, we can generate anonymous cases that are not bound to privacy regulation.

%\textbf{This is an example.} Any text generation application that learns from data runs the risk of producing biased or offensive content reflective of the training data—our work, which learns a language model from song lyrics, is no exception. One approach that we implement is to moderate the words shown to our language model based on a list of keywords3; a downside of this moderation is the potential for increased bias as a side effect of the content filter. Recent work in modeling the intentions of vulgar expressions has shown promise for more nuanced profanity filtering or hate speech detection [12], and as these approaches improve, they present one path toward better automated moderation when working on text generation. In addition to biased or offensive content, the other common ethical concern when working with material like lyrics is the potential for plagiarism. In our setting, one of the reasons we choose to work with arbitrary audio inputs is to explicitly condition the language model with a strong signal which, intuitively, should make it difficult to copy from the training set; still, more work is needed to determine the extent to which the audio conditioning reduces plagiarism.

%\textbf{This is instruction.} Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
%Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages biases in the data. If authors believe this is not applicable to them, authors can simply state this.

%Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}

==> discussion.tex <==
We have demonstrated on MNIST and CLEVR datasets that MSGNet can learn the intrinsic relationship between various objects in a image, and the generations adhere to the semantic and spatial constraints. 

Through experiments on two medical datasets, we have shown that MSGNet can be used to generate samples with object-level annotations for problems where auxiliary information such as object location and identity cannot be easily provided as an input during generation. We demonstrated improvement on a malaria cell detection problem as well as showed that MSGNet could generate good quality samples for brain tumors. The improvements on the Malaria and BrATS segmentation datasets further indicate that such a generative model, providing object level control as well as the annotations, could be a valuable data augmentation tool.

However, it is important to note that we have assumed several simplifications in our current work. For the numerical experiments, we only worked with images containing a few classes. Our VQ-VAE and PixelSNAIL architectures are relatively simple in terms of discriminative power. We argue that the quality of generations can be improved further through several straightforward modifications. First, the discriminative power of our approach can be improved significantly by replacing the current backbone autoencoder with more powerful backbones such as VQ-VAE-2 \cite{Razavi2019iclr}. We believe that increasing the latent size and with that the complexity of the PixelSNAIL model also ensures better generations but at the cost of more computation. Additionally, the background contains valuable information that can aid generations. As opposed to treating the background with just one or two classes, we suggest allowing the model to learn a more discriminative conditioning of the background based on the object labels. That is, an embedding can be build for the background class in every image by considering the object classes within an image.

==> related_work.tex <==
 % \textbf{Image Generation from Scene Graphs}
% Conditional Image Synthesis conditions generation on additional input. GANs can be conditioned on category labels by providing labels as an additional input to both generator and discriminator [10, 35] or by forcing the discriminator to predict the label [37]
% Reed et al. [42] generate images from text using a GAN; Zhang et al. [59] extend this approach to higher resolutions using multistage generation. Related to our approach, Reed et al. generate images conditioned on sentences and keypoints using both GANs [41] and multiscale autoregressive models [43]; in addition to generating images they also predict locations of unobserved keypoints using a separate generator and discriminator operating on keypoint locations.
% Chen and Koltun [6] generate high-resolution images of street scenes from ground-truth semantic segmentation using a cascaded refinement network (CRN) trained with a perceptual feature reconstruction loss [9, 21]; we use their
% CRN architecture to generate images from scene layouts. Related to our layout prediction, Chang et al. have investigated text to 3D scene generation [4, 5]; other approaches
% to image synthesis include stochastic grammars [20], probabalistic programming [27], inverse graphics [28], neural
% de-rendering [55], and generative ConvNets [56].

% - Counter
% Previous works focused on a popular simplified instance
% of the problem described above: scene generation based on
% sentence description [6, 11, 12, 19, 24, 25, 30]. A typical
% sentence description includes partial information on both
% the background and objects, along with details of the objects’
% appearances and scene layout. These frameworks rely
% heavily on the extra relational information provided by the
% sentence. As a result, although these methods manage to
% generate realistic scenes, they tend to ignore learning the
% intrinsic relationships between the objects, prohibiting the
% wide adoption of such models where weaker descriptions
% are provided.




% \textbf{ICLR}
% Having more control over the general image layout can lead to a higher quality of images (\cite{reed2016generative}Reed et al.,
% 2016a; Hong et al., 2018b) and is also an important requirement for semantic image manipulation
% (Hong et al., 2018a; Wang et al., 2018). Approaches that try to exert some control over the image
% layout utilize Generative Adversarial Nets (Goodfellow et al., 2014), Refinement Networks (e.g. Chen
% & Koltun (2017); Xu et al. (2018a)), recurrent attention-based models (e.g. Mansimov et al. (2016)),
% autoregressive models (e.g. Reed et al. (2016c)), and even memory networks supplying the image
% generation process with previously extracted image features (Zhang et al., 2018b).


% [Reed]  Generative adversarial text-to-image synthesis
% [Reed] Generating interpretable images with controllable structure.


% Generative Image Models fall into three recent categories: Generative Adversarial Networks (GANs) [12, 40]
% jointly learn a generator for synthesizing images and a discriminator classifying images as real or fake; Variational
% Autoencoders [24] use variational inference to jointly learn
% an encoder and decoder mapping between images and latent codes; autoregressive approaches [38, 53] model likelihoods by conditioning each pixel on all previous pixels.


Deep generative models such as GANs~\cite{goodfellow2014nips}, VAEs~\cite{kingma2014iclr} and Autoregressive models ~\cite{oord2016icml} are now widely popular for generating synthetic images. In particular, BigGAN \cite{brock2019iclr} and VQ-VAE \cite{Oord2017neurips} have been successful in generating very high-quality realistic images. However, to generate high-fidelity images with more realistic localization of objects, these models need to be conditioned with auxiliary information that contains the notion of spatial and semantic coherency among objects and their respective background. We observe in the literature that this is yet exclusively done with GAN-based models.

% Having more control over the general image layout can lead to a higher quality of images.

% To generate more realistic and complex scenes, image synthesis models can benefit from incorporating
% a notion of localizable objects.

% The same types of objects can appear in many locations in different scales, poses and configurations. This fact can be exploited by separating the questions of “what”
% and “where” to modify the image at each step of computation. In addition to parameter efficiency,
% this yields the benefit of more interpretable image samples, in the sense that we can track what the
% network was meant to depict at each location.
% recent approaches are broadly based on: (a) Variational Auto-Encoders (VAEs) ~\cite{kingma2014iclr,pu2016nips} which uses variational inference to jointly learn an encoder and decoder where the former maps images into latent codes; (b)  learning a generator for generating images and a discriminator predicting images as real or fake; (c) autoregressive models such as Pixel-
% RNN ~\cite{oord2016icml} and PixelCNN ~\cite{van2016nips} synthesize images pixel by
% pixel based on conditional distribution over pixels.

Several models have exploited the use of additional input to condition the image generation process. These include using natural language descriptions ~\cite{mansimov2015iclr,reed2016icml,zhang2017iccv}, image category labels ~\cite{miyato2018iclr,zhang2019icml}, scene graphs ~\cite{johnson2018cvpr, yikang2019nips} and paired or unpaired  source images ~\cite{ huang2018eccv, liu2019iccv}. To gain precise control over the placement of discrete objects in an image, some approaches ~\cite{wang2018cvpr,park2019cvpr} constrain the generation using annotated semantic layouts. Since these approaches are explicitly regularised by conditional inputs, they ignore the intrinsic relationship between objects; this not only puts a large dependency on the quality of auxiliary inputs, but also limits diversity in the generated images. 

 Recent works have proposed generative learning frameworks with broadly a two-step approach: predicting semantic layouts from either text description or scene graph and conditioning image generation on these layouts. 
\mbox{Hinz et al.}~\cite{Hinz2019iclr} proposed a text-to-image generation framework in which spatial ordering of objects are controlled by adding an extra object pathway.
%in both the generator and discriminator. 
Some approaches  only focus on generating semantically coherent layouts given a set of images ~\cite{li2019iclr, jyothi2019iccv}, while others take a scene graph as input ~\cite{johnson2018cvpr, tripathi2019iclrw}.
%as input and later train an image generator independently.
%Others take scene graph as input and generates images by producing an intermediate layout by learning embeddings of nodes  
%In ~\cite{hong2018cvpr}, image captions are used to generate bounding boxes of objects within an image, predict object's shape within the box and finally convert it to an image using an image generator. The follow-up work in~\cite{hong2018nips} enabled the capturing of object shape, object-object interactions, and object-scene relations; making it possible to manipulate images on a more semantic level. 

The work in ~\cite{hong2018cvpr, hong2018nips} enabled the capturing of object shape, object-object interactions, and object-scene relations. Although, the generations of these approaches are still conditioned on layout or textual information at a coarser level. Thus, the problem of limited diversity in the generations prevails here as well. This prohibits the applicability of all these approaches on non-natural images.

Lastly, GANs have been demonstrated to be capable of generating high-quality images to augment the original data, resulting in an increase of classification performance \cite{gansmedicalanalysis2018, brain1}. Nevertheless, the use of GANs involves problems such as mode collapse, unstable training and a lack of diversity. 
% On the other hand, negative log-likelihood models, such as VAEs, assign probabilities to all modes of the data, thereby circumventing these problems. However, despite VAEs offering a more stable training regime, their generations are often more blurry. The authors in \cite{Kwon2019GenerationO3, Han2019CombiningNA} leverage from both VAEs and GANs to alleviate GANs' shortcomings for data augmentation. In addition, although these approaches use segmentation masks to correctly generate an image according to its mask; the semantic relationship between the objects and background  are not fully exploited. Comparably, in \cite{bloodcellgan2019}, a GAN-based pipeline is proposed to generate red blood cell images along with the instance segmentation masks. But the segmentation masks are specific for red blood cell images and this approach could not be used for more complicated layouts. 

% Both these approaches ~\cite{hong2018cvpr,hong2018nips} require detailed  instance segmentation masks of objects while training its object shape generator which is unscalable and labor intensive, especially for non-natural images.





% The LayoutVAE \cite{jyothi2019iccv} synthesizes semantic layout of a scene given a set of labels.  However, a non-natural  layout has
% several fundamental differences to a natural scene layout.
% The demands for relationship and alignment among components are strict 






% How to feed conditional information to
% a GAN model has been studied in various ways. In [9],
% [16], the conditional information are encoded to a vector,
% concatenated with noise, and then passed to the generator.
% In [6], projection-based methods, which incorporate conditional
% information to the discriminator by inner product
% between feature and learned class embedding, effectively
% improve the quality of class conditional image generation.
% In [16], [17], [41], conditional information is utilized by the
% discriminator using simple concatenation with the input or
% intermediate feature maps. In [5], [15], [42], [43], conditional
% information is provided to the generator by conditional
% gains and bias in the Batch Normalization [29] layers.

% In layout-to-image, the layout that a synthesized image
% needs to satisfy consists of labeled bounding boxes configured
% in an image lattice (e.g., 256  256 pixels). The style
% of a synthesized image refers to structural and appearance
% variations at both image and object levels, which is often
% encoded by some latent codes. Generating images from a
% spatial layout represents a sweet spot in conditional image synthesis. Spatial layouts are usually used as intermediate
% representations for other conditional image synthesis
% tasks such as text-to-image [17], [21] and scene-graph-toimage
% [18], [19]. And, layouts are more flexible, less constrained
% and easier to collect than other conditions such
% as semantic segmentation maps [11], [14]. The generative learning task of layout-to-image was
% recently proposed and only a few work have been proposed
% in the very recent literature [18], [19], [20], [23]. Although
% relatively new, it has been well recognized in the computer
% vision community. For example, the work (Grid2Im) by
% Ashua andWolf [19] won the best paper honorable mentions
% at ICCV 2019. The layout-to-image task was emerged under
% the context of remarkable progress made in conditional
% image synthesis with relatively less complicated conditions
% such as the class-conditional image synthesis in ImageNet
% by the BigGAN [5], and the amazing style control for specific


% A typical
% sentence description includes partial information on both
% the background and objects, along with details of the objects’
% appearances and scene layout. These frameworks rely
% heavily on the extra relational information provided by the
% sentence. As a result, although these methods manage to
% generate realistic scenes, they tend to ignore learning the
% intrinsic relationships between the objects, prohibiting the
% wide adoption of such models where weaker descriptions
% are provided. 
 
 





% Generating images from text descriptions has recently
% drawn a lot of attention from the research community. Formulating the task as a conditional image generation problem, various approaches have been proposed based on Variational Auto-Encoders (VAE) [16], auto-regressive models [23], optimization techniques [18], etc. Recently, approaches based on conditional Generative Adversarial Network (GAN) [7] have shown promising results in text-toimage synthesis [22, 24, 36, 6, 4]. Reed et al. [22] proposed
% to learn both generator and discriminator conditioned on
% text embedding. Zhang et al. [36] improved the image quality by increasing image resolution with a two-stage GAN.
% Other approaches include improving conditional generation by augmenting text data with synthesized captions [6],
% or adding conditions on class labels [4]. Although these
% approaches have demonstrated impressive generation results on datasets of specific categories (e.g., birds [35] and
% flowers [19]), the perceptual quality of generation tends to
% substantially degrade on datasets with complicated images
% (e.g., MS-COCO [14]).



% scene generation based on
% sentence description [6, 11, 12, 19, 24, 25, 30]. A typical
% sentence description includes partial information on both
% the background and objects, along with details of the objects’
% appearances and scene layout. These frameworks rely
% heavily on the extra relational information provided by the
% sentence. As a result, although these methods manage to
% generate realistic scenes, they tend to ignore learning the
% intrinsic relationships between the objects, prohibiting the
% wide adoption of such models where weaker descriptions
%are provided.

==> results-coco.tex <==
MS-coco experiment to be compared with stackedGAN stackedGAN+objectpathways. Both methods are to be implemented without the text part.

\begin{table}
  \caption{Results on MS-COCO dataset.}
  \label{table-mscoco-exp}
  \centering
  \begin{threeparttable}[t]
  \centering
  \begin{tabular}{l | c | l | l}
  \toprule
    %\cmidrule(r){1-2}
    Model  & Resolution     & IS $\uparrow$ & FID $\downarrow$\\
    \midrule
    AttnGAN \cite{}\tnote{1} & $N \times N$  & - & -     \\
    VQVAE-2 \cite{}\tnote{2}     & $N \times N$ & - & -      \\
    AttnGAN + \emph{Object Pathways} \cite{}\tnote{1}    & $N \times N$ & - & -  \\
    VQVAE-2 + conditioning (first one)\tnote{2} & $N \times N$ & - & -\\
    MOGNet (ours) & $N \times N$ & - & - \\
    \bottomrule
  \end{tabular}
  \begin{tablenotes}
  \item[1] footnote 1
  \item[2] footnote 2
  \end{tablenotes}
  \end{threeparttable}
\end{table}

==> results-mnist-clevr.tex <==

\begin{comment}
\begin{figure}
\begin{minipage}{0.5\textwidth}
\centering
\begin{subfigure}{1\textwidth}
\centering
\includegraphics[scale=0.58]{images/mnist_tests/semantic/gan/1.png}
\includegraphics[scale=0.58]{images/mnist_tests/semantic/gan/2.png}
\includegraphics[scale=0.58]{images/mnist_tests/semantic/vqvae/multiple_1.png}
\includegraphics[scale=0.58]{images/mnist_tests/semantic/vqvae/viol1.png}
\includegraphics[scale=0.58]{images/mnist_tests/semantic/gan/fail3.png}

\end{subfigure}
\begin{subfigure}{1\textwidth}
\centering
\includegraphics[scale=0.58]{images/mnist_tests/semantic/vqvae/gen1.png}
\includegraphics[scale=0.58]{images/mnist_tests/semantic/vqvae/gen2.png}
\includegraphics[scale=0.58]{images/mnist_tests/semantic/vqvae/4.png}
\includegraphics[scale=0.58]{images/mnist_tests/semantic/vqvae/00.png}
\includegraphics[scale=0.58]{images/mnist_tests/semantic/vqvae/gen5.png}
\end{subfigure}
\begin{subfigure}{1\textwidth}
\centering
\includegraphics[scale=0.58]{images/mnist_tests/semantic/mognet/0_8.png}
\includegraphics[scale=0.58]{images/mnist_tests/semantic/mognet/5_1.png}
\includegraphics[scale=0.58]{images/mnist_tests/semantic/mognet/7_2.png}
\includegraphics[scale=0.58]{images/mnist_tests/semantic/mognet/6_4_fail.png}
\includegraphics[scale=0.58]{images/mnist_tests/semantic/mognet/5_1_2.png}
\end{subfigure}
\captionsetup{width=.97\linewidth}
\addtocounter{figure}{-1}
\captionof{figure}{Generations obtained with cGAN\cite{Hinz2019iclr} (top), cVQ-VAE\cite{Oord2017neurips} (middle) and MSGNet (bottom). Only following pairs were allowed: \{6,4\}, \{7,2\}, \{5,1\}, \{8,0\} and \{9,3\}}
\label{fig_mnist_semantic}
\end{minipage}
\begin{minipage}{0.5\textwidth}
\centering
\begin{subfigure}{1\textwidth}
\centering
\includegraphics[scale=0.58]{images/mnist_tests/spatial/gan/ex1.png}
\includegraphics[scale=0.58]{images/mnist_tests/spatial/gan/ex5.png}
\includegraphics[scale=0.58]{images/mnist_tests/spatial/gan/ex_2.png}
\includegraphics[scale=0.58]{images/mnist_tests/spatial/gan/ex_3.png}
\includegraphics[scale=0.58]{images/mnist_tests/spatial/gan/ex_6.png}

\end{subfigure}
\begin{subfigure}{1\textwidth}
\centering
\includegraphics[scale=0.14]{images/mnist_tests/spatial/mognet/mnist2.png}
\includegraphics[scale=0.14]{images/mnist_tests/spatial/vqvae/goodexvqvae.png}
\includegraphics[scale=0.14]{images/mnist_tests/spatial/vqvae/mnistviolates1.png}
\includegraphics[scale=0.14]{images/mnist_tests/spatial/vqvae/mnistviolates6.png}
\includegraphics[scale=0.14]{images/mnist_tests/spatial/vqvae/mnistviolates3.png}
\end{subfigure}
\begin{subfigure}{1\textwidth}
\centering
\includegraphics[scale=0.14]{images/mnist_tests/spatial/vqvae/mnist1.png}
\includegraphics[scale=0.14]{images/mnist_tests/spatial/mognet/mnist3.png}
\includegraphics[scale=0.14]{images/mnist_tests/spatial/mognet/mnist4.png}
\includegraphics[scale=0.14]{images/mnist_tests/spatial/mognet/mnist5.png}
\includegraphics[scale=0.14]{images/mnist_tests/spatial/mognet/mnist6.png}
\end{subfigure}
\captionsetup{width=.95\linewidth}
\addtocounter{figure}{-1}
\captionof{figure}{Generations obtained with cGAN \cite{Hinz2019iclr} (top), cVQ-VAE \cite{Oord2017neurips} (middle)  and our MSGNet (bottom). Objects were allowed to occur in only the upper-half of the images.}
\label{fig_mnist_spatial}

\end{minipage}
\end{figure}
\end{comment}

\begin{figure}[h]
\centering
\begin{subfigure}{0.49\textwidth}
\centering
\includegraphics[scale=0.24]{images/clevr_tests/semantic/mognet/layout_10.png}\hspace{-0.2em}
\includegraphics[scale=0.24]{images/clevr_tests/semantic/mognet/layout_11.png}\hspace{-0.2em}
\includegraphics[scale=0.168]{images/clevr_tests/semantic/vqvae/viol.jpg}\hspace{-0.2em}
\includegraphics[scale=0.127]{images/clevr_tests/semantic/vqvae/vqvae4.jpeg}
\caption{Pre-MSGNet}
\end{subfigure}
\begin{subfigure}{0.49\textwidth}
\centering
\includegraphics[scale=0.24]{images/clevr_tests/semantic/mognet/layout_1.png}\hspace{-0.2em}
\includegraphics[scale=0.24]{images/clevr_tests/semantic/mognet/layout_3.png}\hspace{-0.2em}
\includegraphics[scale=0.24]{images/clevr_tests/semantic/mognet/layout_5.png}\hspace{-0.2em}
\includegraphics[scale=0.24]{images/clevr_tests/semantic/mognet/layout_6.png}
\caption{MSGNet}
\end{subfigure}
\caption{Example generations on CLEVR dataset. Added constraint was that each image should contain one object positioned at the center, no object at the extreme corners, and reflections should be coherent. Pre-MSGNet violates the constraint when incorrect auxiliary information is provided.}
\label{fig_clevr_semantic}
\end{figure}
% In this section, we study the efficacy of our model in capturing the semantic and spatial coherencies in the underlying data distribution. 
The goal of the spatial and semantic coherency experiments is to identify how well the constraints are satisfied in the generations of the model. We compare the generations with VQ-VAE \cite{Oord2017neurips} adapted with layout conditioning (referred further as cVQ-VAE) and GAN with object pathways (obj-cGAN) \cite{Hinz2019iclr}. 

%Further, to study spatial coherency on Multi-MNIST, we constrain that every image in the training set contains 3 digits that occur strictly in the upper half of image. This implies that any generated image that contains digits in the lower half will be deemed as invalid.  As shown in Fig. \ref{fig_mnist_spatial}, MSGNet adheres to the spatial constraint in the generations. On the other hand, the two explicitly conditioned methods, cVQ-VAE and obj-cGAN, violate the spatial constraint and generate digits in the lower half of the image when provided with wrong input. Among the two, cVQ-VAE seems to reject the generation of digits in the lower half to a better extent, and leaves almost blank regions instead. Nevertheless, our MSGNET qualitatively outperforms the other two methods in terms of abiding by the constraints.

%We study semantic and spatial coherency on CLEVR dataset using a single experiment. The imposed constraints require that every image should contain one object centered in the image, and another object randomly positioned around it so that the reflections are visible. The light source is positioned in a manner that whenever the two objects are close, the reflection of one is visible on the other. In Fig. \ref{fig_clevr_semantic}, we see that both MSGNet as well as cVQ-VAE, capture the reflections very well. As already seen in \mbox{Fig. \ref{fig_clevr_basic}}, obj-cGAN fails to generate coherent shadows as well as its generations were relatively inferior. Hence, we do not use obj-cGAN in this experiment. We observed that cVQ-VAE, when given wrong object locations, generated semantically coherent samples that are visually plausible. For example, it could generate samples that do not contain any object positioned at the center. Similar to the previous experiment, our MSGNet always generates acceptable samples%, since the intrinsic relationships between objects are implicitly learned. 

% need to fix this last part

%The observations from the experiment on the CLEVR dataset translate to the fact that explicitly conditioned models require very accurate and tailored auxiliary information, and the diversity of their generations is restricted by the expressivity of the provided weak descriptions. For non-natural images such as medical images, such conditional image generation approaches would not be preferred. MSGNet learns the intrinsic relationships from directly the images and is thus better suited for natural images. This is validated through the next experiments.


==> short_discussion.tex <==
We demonstrated that MSGNet learns the intrinsic relationship between various objects in a image, and the generations adhere to the semantic constraints. This was useful with non-natural images such as in a Malaria-cell detection problem and in brain tumor segmentation. 
However, it is important to note that we have assumed several simplifications in our current work. Our VQ-VAE and PixelSNAIL architectures are relatively simple in terms of discriminative power. The discriminative power of our approach can be improved significantly at the cost of more computation by replacing the current backbone autoencoder with more powerful backbones such as VQ-VAE-2 \cite{Razavi2019iclr} and by increasing the latent size to ensure better generations.
